SCOTCH and SODA: A Transformer Video Shadow Detection Framework

Shadows in videos are difficult to detect because of the large shadow deformation between frames. In this work, we argue that accounting for shadow deformation is essential when designing a video shadow detection method. To this end, we introduce the shadow deformation attention trajectory (SODA), a new type of video self-attention module, specially designed to handle the large shadow deformations in videos. Moreover, we present a new shadow contrastive learning mechanism (SCOTCH) which aims at guiding the network to learn a unified shadow representation from massive positive shadow pairs across different videos. We demonstrate empirically the effectiveness of our two contributions in an ablation study. Furthermore, we show that SCOTCH and SODA significantly outperforms existing techniques for video shadow detection. Code is available at the project page: https://lihaoliu-cambridge.github.io/scotch_and_soda/

==> equation/equation_1.tex <==
\begin{equation}
\begin{aligned} \label{eq:eq1_transformer_layer}
    y &= \textrm{MSA}(\textrm{LN}(z)) + z, \\
    z' &= \textrm{MLP}(\textrm{LN}(y)) + y
\end{aligned}
\end{equation}
where $z'$ is the learned representation of the 1D sequential embeddings, LN is a layer norm operation, MSA is the multi-head self-attention module, and MLP is the MLP layers.
%

==> equation/equation_2.tex <==
\begin{equation}
\begin{aligned} \label{eq:eq2_self_attention}
    \textrm{Attention}(q, k, v) & = \textrm{Softmax}\bigg(\frac{q\cdot k^T}{\sqrt{n}}\bigg)\cdot v \\
\end{aligned}
\end{equation}
%

==> equation/equation_3.tex <==
\begin{equation}
\begin{aligned} \label{eq:eq3_pixelwise_self_attention}
    y_{s t}=\sum_{s^{\prime} t^{\prime}} v_{s^{\prime} t^{\prime}} \cdot \frac{\exp \langle q_{s t}, k_{s^{\prime} t^{\prime}} \rangle}{\sum_{\bar{s} \bar{t}} \exp \langle q_{s t}, k_{\bar{s} \bar{t}} \rangle}
\end{aligned}
\end{equation}
where $st, s^{\prime} t^{\prime}, \bar{s} \bar{t} \in \{1, 2, 3, ..., n\}$ denotes one position in the 1D sequence, and $q_{st}, k_{st}, v_{st}$ comes from the $st$ position of $q, k, v$, respectively. For brevity, the notation is slightly abused by omitting the softmax and temperature parameter $\sqrt{n}$.
%


==> equation/equation_4.tex <==
\begin{equation}
\begin{aligned} \label{eq:eq4_traj_attention_part1}
    \tilde{y}_{s t t^{\prime}}=\sum_{s^{\prime}} v_{s^{\prime} t^{\prime}} \cdot \frac{\exp \langle q_{s t}, k_{s^{\prime} t^{\prime}} \rangle}{\sum_{\bar{s}} \exp \langle q_{s t}, k_{\bar{s} t^{\prime}} \rangle}
\end{aligned}
\end{equation}
where $\hat{y}_{stt^{\prime}}$ represents the spatial attentions (trajectories) between two frames that indicate how the object in $s$ moves from frame $t$ to frame $t^{\prime}$.
%

==> equation/equation_56.tex <==
\begin{equation}
\begin{aligned} \label{eq:eq5_traj_attention_new_qkv}
    \tilde{q}_{s t}=\tilde{w}_{q} \cdot \tilde{y}_{s t t}, \; \tilde{k}_{s t t^{\prime}}=\tilde{w}_{k} \cdot \tilde{y}_{s t t^{\prime}}, \; \tilde{v}_{s t t^{\prime}}=\tilde{w}_{v} \cdot \tilde{y}_{s t t^{\prime}}.
\end{aligned}
\end{equation}
where $\tilde{y}_{s t t}$ contains spatial connection from $st$ to the same frame $t$, and $\tilde{q}_{s t}$ corresponds to the trajectory reference point $st$, which is used to aggregate information across the new
time/trajectory dimension:
\begin{equation}
\begin{aligned} \label{eq:eq6_traj_attention_part2}
    \tilde{y}_{s t}=\sum_{t^{\prime}} \tilde{v}_{s t t^{\prime}} \cdot \frac{\exp \langle \tilde{q}_{s t}, \tilde{k}_{s t t^{\prime}} \rangle}{\sum_{\bar{t}} \exp \langle \tilde{q}_{s t}, \tilde{k}_{s t \bar{t}} \rangle}
\end{aligned}
\end{equation}
where $\tilde{y}_{st}$ is the trajectory attention output. By computing the intra-frame attention, the complete trajectory attention is capable of lending a realistic inductive bias to the model that can boost the video processing performance.
%
